Investigation of Inward-Outward Ring Permanent Magnet Array for Portable Magnetic Resonance Imaging (MRI)

Permanent magnet array (PMA) is a popular option to provide the main magnetic field in a dedicated portable magnetic resonance imaging (MRI) system because it does not need power or a cooling system and has a much stronger field strength compared to a resistive magnet. Aside from the popular Halbach array that has a transversal field direction, the Inward-Outward ring (IO ring) array is a promising candidate that offers a longitudinal field direction with various design and engineering possibilities. In this article, a thorough study of IO ring arrays is conducted by examining the relation between the design parameters and its field patterns, its variants that lead to different applications and their properties. A detailed comparison between an IO ring array and Halbach array was conducted and reported. Moreover, the feasibility of building an IO ring array in a lab is demonstrated. The investigations strongly indicate that IO ring is a promising candidate that can offer high and homogeneous fields or a desired field pattern to portable MRI systems. With a longitudinal field direction, an IO ring array opens up opportunities to adopt MRI advanced technology and techniques in a portable system to improve image quality and shorten scan time.

==> fig_est_four.tex <==
\begin{figure}[t]
\centering
\begin{center}
\newcommand{\patchSize}{2.45cm}
\scriptsize
\setlength\tabcolsep{0.1cm}
\includegraphics[width=0.9\linewidth]{figures/Fig_est_four_1.jpg}\\
(a)\hspace{0.43\linewidth}(b)\\    \includegraphics[width=0.9\linewidth]{figures/Fig_est_four_2.jpg}\\
(c)\hspace{0.43\linewidth}(d)\\ 	
\end{center}
\caption{The estimated (black) and calculated (red) $B_\text{z}$ magnetic field component at the origin while sweeping the four parameters: (a) $R_\text{in}$, (b) $Z_\text{in}$, (c) $h_\text{r}$, and (d) $h_\text{z}$. The corresponding parameters were set accordingly with Fig.\,\ref{fig:result_four}.}
\label{fig:est_four}
\end{figure}

==> fig_field_asym_z60.tex <==
\begin{figure}[t]
\centering
\begin{center}
\newcommand{\patchSize}{2.45cm}
\scriptsize
\setlength\tabcolsep{0.1cm}
\includegraphics[width=0.7\linewidth]{figures/Fig_field_asym_z60_1.jpg}\\
(a)\hspace{0.3\linewidth}(b)\\    \includegraphics[width=0.7\linewidth]{figures/Fig_field_asym_z60_2.jpg}\\
(c)\hspace{0.3\linewidth}(d)\\ 	
\end{center}
\caption{The $B_\text{z}$ magnetic field component at (a) $z=-100$ mm, (b) $z=0$ mm and (c) $z=50$ mm for the asymmetric IO ring array in Fig.\,\ref{fig:field_asym_ring} with $R_\text{diff}=60$ mm. (d) The corresponding 1D field plot along the $x$-direction with $y=0$.}
\label{fig:asym_z60}
\end{figure}

==> tab_labIO_slices.tex <==
\begin{table}[ht]
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{$z$ {[}mm{]}} & \textbf{mean($B_\text{z}$) {[}mT{]}} & \textbf{RF Bandwidth {[}\%{]}} & \textbf{$R^2$} \\ \hline
0                     & 39.3                                 & 8.90                           & 0.949          \\ \hline
20                    & 39.7                                 & 9.22                           & 0.984          \\ \hline
35                    & 40.3                                 & 8.01                           & 0.968          \\ \hline

\end{tabular}
\end{center}
\caption{The average field strength, RF bandwidth, and field linearity represented by the determination coefficient $R^2$ at $z=0, 20, 35$\,mm for the PMA in Fig.\,\ref{fig:labIO_overview}.}
\label{tab:labIO_slices}
\end{table}

==> tab_n_bar_field.tex <==
\begin{table}[ht]
\begin{center}
\begin{scriptsize}
\begin{tabular}{|l|l|ll|ll|ll|}
\hline
\multirow{2}{*}{\textbf{$n_\text{bar}$}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}$a$\\ {[}mm{]}\end{tabular}}} & \multicolumn{2}{l|}{\textbf{mean($B_\text{z}$) {[}mT{]}}}                      & \multicolumn{2}{l|}{\textbf{Inhomogeneity {[}\%{]}}}        & \multicolumn{2}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Periphery-center\\ gradient {[}mT/m{]}\end{tabular}}} \\ \cline{3-8} 
                                         &                                                                                          & \multicolumn{1}{l|}{\textbf{$z=0$ mm}} & \textbf{$z=10$ mm}                    & \multicolumn{1}{l|}{\textbf{$z=0$ mm}} & \textbf{$z=10$ mm} & \multicolumn{1}{l|}{\textbf{$z=0$ mm}}                          & \textbf{$z=10$ mm}                         \\ \hline
3                                        & 346.4                                                                                    & \multicolumn{1}{l|}{33.2}              & 32.9 ($\downarrow$0.9\%) & \multicolumn{1}{l|}{20.7}              & 22.6               & \multicolumn{1}{l|}{113.3}                                      & 123.4                                      \\ \hline
4                                        & 200                                                                                      & \multicolumn{1}{l|}{37.8}              & 37.5 ($\downarrow$0.8\%) & \multicolumn{1}{l|}{21.0}              & 22.8               & \multicolumn{1}{l|}{109.1}                                      & 126.7                                      \\ \hline
6                                        & 115.5                                                                                    & \multicolumn{1}{l|}{40.7}              & 40.6 ($\downarrow$0.2\%) & \multicolumn{1}{l|}{17.6}              & 20.4               & \multicolumn{1}{l|}{119.8}                                      & 138.1                                      \\ \hline
8                                        & 82.8                                                                                     & \multicolumn{1}{l|}{41.6}              & 41.6 (-)                              & \multicolumn{1}{l|}{16.0}              & 19.1               & \multicolumn{1}{l|}{109.7}                                      & 131.0                                      \\ \hline
12                                       & 53.6                                                                                     & \multicolumn{1}{l|}{42.2}              & 42.2 (-)                              & \multicolumn{1}{l|}{14.9}              & 18.2               & \multicolumn{1}{l|}{104.9}                                      & 127.7                                      \\ \hline
16                                       & 39.8                                                                                     & \multicolumn{1}{l|}{42.4}              & 42.4 (-)                              & \multicolumn{1}{l|}{14.5}              & 17.9               & \multicolumn{1}{l|}{102.7}                                      & 126.2                                      \\ \hline
continuous                               & N/A                                                                                      & \multicolumn{1}{l|}{44.1}              & 44.0 ($\downarrow$0.2\%) & \multicolumn{1}{l|}{14.5}              & 17.8               & \multicolumn{1}{l|}{106.3}                                      & 130.7                                      \\ \hline
\end{tabular}
\end{scriptsize}
\end{center}
\caption{The average field strength, inhomogeneity, and gradient strength from periphery to the center at $z=0$ and 10 mm for $n_\text{bar}=0,3,4,6,8,12,16$ as in Fig.\,\ref{fig:result_nbar}\,(a) and (b).}
\label{tab:nbar_field}
\end{table}
